Spin Dynamics of Complex Oxides, Bismuth-Antimony Alloys, and Bismuth Chalcogenides

This thesis predicts that two types of material families could be a solution to the challenges in spintronics: complex oxides and bismuth based materials. We derive a general approach for constructing an effective spin-orbit Hamiltonian, which applies to all nonmagnetic materials. We also verify this formalism through comparisons with other approaches for III-V semiconductors. Its general applicability is illustrated by deriving the spin-orbit interaction and predicting spin lifetimes for strained SrTiO$_3$ and a two-dimensional electron gas (such as at the LaAlO$_3$/SrTiO$_3$ interface). Our results suggest robust spin coherence and spin transport properties in SrTiO$_3$ related materials. In the second part, we calculate intrinsic spin Hall conductivities for Bi$_{1-x}$Sb$_x$ semimetals with strong spin-orbit couplings, from the Kubo formula and using Berry curvatures evaluated from a tight-binding Hamiltonian. Nearly crossing bands with strong spin-orbit interaction generate giant spin Hall conductivities in these materials, ranging from 474 ($\hbar/e)( \Omega^{-1}cm^{-1}$) for bismuth to 96($\hbar/e)( \Omega^{-1}cm^{-1}$) for antimony; the value for bismuth is more than twice that of platinum. The large spin Hall conductivities persist for alloy compositions corresponding to a three-dimensional topological insulator state, such as Bi$_{0.83}$Sb$_{0.17}$. The spin Hall conductivity could be changed by a factor of 5 for doped Bi, or for Bi$_{0.83}$Sb$_{0.17}$, by changing the chemical potential, suggesting the potential for doping or voltage tuned spin Hall current. We also calculate intrinsic spin Hall conductivities of Bi$_2$Se$_3$ and Bi$_2$Te$_3$ topological insulators from an effective tight-binding Hamiltonian. We conclude that bismuth-antimony alloys and bismuth chalcogenides are primary candidates for efficiently generating spin currents through the spin Hall effect.

==> publicAbstract.tex <==
%Prior to your first thesis deposit, replace this text with the text of your public abstract.  The text of this abstract should be double spaced and each new paragraph should be indented.  The text may be altered between first and final deposits.   \\
%This abstract is required for all thesis/dissertations. 
%The public abstract is to be placed at this point in your first and final deposits  and submitted via this web form at final deposit. (https://www.grad.uiowa.edu/public-abstracts)  This abstract may be up to 250 words and should be written for a non-academic lay audience.  In writing your public abstract, avoid jargon and technical language as much as possible. \\
%
%The ability to communicate research simply and clearly is an important skill when interviewing for faculty positions, as well as for positions in industry and alt-ac sectors. The public abstract helps convey ideas beyond one’s immediate academic circle, facilitating communication with colleagues who do different kinds of work and possess different dimensions of training.\\
%
%Think of your public abstract as your “elevator pitch” or what you might tell someone who asks, “What is your thesis about?”  You may only have a few minutes to explain it to them while keeping their attention and using terminology you are sure they will understand without further lengthy explanation.    
Spintronics is an emerging field of condensed matter physics which aims to change the functioning principles of electronic devices. Spintronics offers a variety of opportunities for electron and nuclear spin, which are intrinsic properties of subatomic particles, to carry information and perform computations. This new paradigm for computer chips and memories promises more efficient devices with much higher speed, less power consumption, nonvolatility and even quantum computation. Recent progress in physics and materials engineering holds the promise of building such spintronic devices shortly. However, there are still several challenges that should be addressed. Two types of materials that are studied in this thesis aim to help solve two fundamental problems of spintronics: bismuth based alloys and topological insulators that can efficiently generate a spin current and complex perovskite oxides which can retain the polarization of spins for long times.

Complex oxides with a variety of properties and design flexibility are of particular interest for spintronic applications. In this thesis, we derive an effective spin-orbit Hamiltonian and calculate spin lifetimes of \LAOSTO interfaces and \STO crystals. Our calculations show that these oxides have exceptionally long spin lifetimes even at room temperature. The second part of this work focuses on bismuth-based materials, such as bismuth-antimony alloys and bismuth chalcogenides, and proves that they are excellent materials for the generation of currents with full spin polarization. In conclusion, both \STO heterostructures and bismuth-related alloys and chalcogenides are promising candidates for materials to be used in spintronic transistors. 


==> thesisAbstract.tex <==
%Prior to your first thesis deposit, replace this text with the text of your scientific/ scholarly abstract.  The text of this abstract should be double spaced and each new paragraph should be indented.  This text may be altered between first and final deposits.  \\
%This abstract is required for everyone except DMA and MFA students.
%This text may be altered between first and final deposits. 
The emerging field of spintronics relies on the manipulation of electron spin in order to use it in spin-based electronics. Such a paradigm change has to tackle several challenges including finding materials with sufficiently long spin lifetimes and materials which are efficient in generating pure spin currents. This thesis predicts that two types of material families could be a solution to the aforementioned challenges: complex oxides and bismuth based materials. 

We derived a general approach for constructing an effective spin-orbit Hamiltonian which is applicable to all nonmagnetic materials. This formalism is useful for calculating spin-dependent properties near an arbitrary point in momentum space. We also verified this formalism through comparisons with other approaches for III-V semiconductors, and its general applicability is illustrated by deriving the spin-orbit interaction and predicting spin lifetimes for strained \STO and a two-dimensional electron gas in \STO (such as at the \LAOSTO interface). Our results suggest robust spin coherence and spin transport properties in \STO related materials even at room temperature.

In the second part of the study we calculated intrinsic spin Hall conductivities for \BiSb semimetals with strong spin-orbit couplings, from the Kubo formula and using Berry curvatures evaluated throughout the Brillouin zone from a tight-binding Hamiltonian. Nearly crossing bands with strong spin-orbit interaction generate giant spin Hall conductivities in these materials, ranging from 474 (($\hbar/e) \Omega^{-1}cm^{-1}$) for bismuth to 96(($\hbar/e) \Omega^{-1}cm^{-1}$) for antimony; the value for bismuth is more than twice that of platinum. The large spin Hall conductivities persist for alloy compositions corresponding to a three-dimensional topological insulator state, such as Bi$_{0.83}$Sb$_{0.17}$. The spin Hall conductivity could be changed by a factor of 5 for doped Bi, or for Bi$_{0.83}$Sb$_{0.17}$, by changing the chemical potential by 0.5 eV, suggesting the potential for doping or voltage tuned spin Hall current. We have also calculated intrinsic spin Hall conductivities of Bi$_2$Se$_3$ and Bi$_2$Te$_3$ topological insulators from an effective  tight-binding Hamiltonian including two nearest-neighbor interactions. We showed that both materials exhibit giant spin Hall conductivities calculated from the Kubo formula in linear response theory and the clean static limit. We conclude that bismuth-antimony alloys and bismuth chalcogenides are primary candidates for efficiently generating spin currents through the spin Hall effect.

